SPRK: A Low-Cost Stewart Platform For Motion Study In Surgical Robotics

To simulate body organ motion due to breathing, heart beats, or peristaltic movements, we designed a low-cost, miniaturized SPRK (Stewart Platform Research Kit) to translate and rotate phantom tissue. This platform is 20cm x 20cm x 10cm to fit in the workspace of a da Vinci Research Kit (DVRK) surgical robot and costs $250, two orders of magnitude less than a commercial Stewart platform. The platform has a range of motion of +/- 1.27 cm in translation along x, y, and z directions and has motion modes for sinusoidal motion and breathing-inspired motion. Modular platform mounts were also designed for pattern cutting and debridement experiments. The platform's positional controller has a time-constant of 0.2 seconds and the root-mean-square error is 1.22 mm, 1.07 mm, and 0.20 mm in x, y, and z directions respectively. All the details, CAD models, and control software for the platform is available at github.com/BerkeleyAutomation/sprk.

==> 4-data.tex <==
\iffalse

\section{Expert Surgeon Demonstrations}
In June 2016, co-author and expert cardiac surgeon Dr. W. Douglas Boyd performed an FLS tasks (pattern cutting) on the Stewart platform.
The experimental setup is depicted in Figure \ref{d_boyd_teleop}.
We recorded trajectory data from these tasks at 90 measurements per second.
This data consisted of the end effector pose of each of the two DVRK arms, and video from the endoscope.
%We focus on the cutting task in this paper and present some initial analysis of this dataset.

\begin{figure}[b]
\centering
\includegraphics[width=0.8\columnwidth]{figures/teleoperation2.png}
\caption{ The experimental setup for the teleoperation data collected from Dr. Boyd. (1) an FLS task was set up on the Stewart platform centered in the workspace, (2) the DVRK, (3) the endoscope camera provided a top down view of the of the workspace. \label{d_boyd_teleop} }
\end{figure}


\subsection{Experiment and Analysis}
In experiment 1, Dr. Boyd cut along a 10 cm line under three types of motion: (1a) no movement, (1b) 0.51 cm, 0.5 Hz sinusoidal lateral movement, and (1c) $10^{o}$, 0.5 Hz rotational movement.
We hypothesized that the surgeon would apply some form of predictive control, and try to compensate for the motion by anticipating where the platform would be.
After running the experiment, we noticed that Dr. Boyd did not track the platform in his control strategy.
Instead, he timed the period of the platform's movement, cutting at the lowest velocity times, i.e, minima and maxima.
This behavior is evident in trajectories with both the rotational and translational motions -- but most pronounced in the rotational motions (Figure \ref{dataDBoyd}).
There was no appreciable reduction in cutting accuracy when Dr. Boyd cut on the moving platform.



\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figures/d_boyd_trajectories.png}
\caption{Surgeon data from one trial period of experiment 1. Results show the distance along the gauze (12 cm) that was cut over time for the platform with (1a) no motion, (1b) lateral movement, (1c) rotational movement. \label{dataDBoyd} }
\setlength\intextsep{0pt}
\end{figure}


Figure \ref{dataDBoyd} plots the the distance cut along the line as a function of time. 
Dr. Boyd completed the baseline task (1a) without any movement in 67 seconds. 
With lateral movement (1b) the task was completed in 139 seconds.
For the rotational movement (1c) the task was completed in 164 seconds.
%The interesting aspect about this result is that it is clearly a sub-optimal policy with respect to time.
Waiting for the low-velocity periods results in nearly 3x longer for cutting the entire line with the rotational movements and more than 2x with the translational movements.
%If the surgeon could track the platform accurately, he would clearly want to do this.
%The natural question is whether we can automate this tracking to optimize this.
%Surprisingly, the next section shows that accurately tracking a moving target for cutting is quite challenging in the presence of variable control latencies and estimation error.


\fi

==> 5-control.tex <==
\iffalse

\section{Control Modes For Cutting}
This section describes the task and 3 control modes for surgical cutting on the Stewart platform.

\begin{figure}[b]
    \includegraphics[width=\columnwidth]{figures/experimental-setup.png}
    \caption{An exploded view of the experimental setup, which is a simplification of the FLS pattern cutting task to evaluate different control architectures. (1) a silicone phantom base, (2) standard FLS surgical gauze marked with a straight 10cm line, (3) tension is provided by standard dissection pins.  \label{exp-setup} }
    \renewcommand{\bottomfraction}{0.25}
\end{figure}

\subsection{Surgical Pattern Cutting Task}
Fundamentals of Laparoscopic Surgery (FLS) is a standard
training regimen for medical students in laparoscopic
surgery; it consists of a suite of five subtasks that increase in
complexity. The second subtask in this suite is called ``Pattern Cutting''. This subtask features a 50 mm diameter,
2 mm thick circular pattern marked on a 10 cm $\times$ 10 cm square of surgical gauze suspended by clips. 
%We assume that the circle lies in the horizontal plane. 
%The subtask is complete once the circle has been cut from the surrounding gauze.
%The FLS suite states that deviations under 2 mm from the line are not penalized.
%We consider a generalization of this task where open and closed contours can be cut.
%This task involves coordinating two arms: the cutting arm which cuts along the contour, and the tensioning arm that holds the gauze in tension while it is being cut.

In prior work, we explored automating the circle cutting task in a static setting ~\cite{murali2015learning, thananjeyanmultilateral}.
We consider a single-arm simplification of this task in a dynamic setting using the Stewart platform (Figure \ref{exp-setup}).
The task includes cutting along a 10 cm straight line while the platform moves under 2.5 cm, 0.2 Hz sinusoidal movements.
Tension is provided by pre-fixed dissection pins and for safety the setup is mounted on a silicone flesh phantom.

\iffalse
\begin{figure}[t]
\includegraphics[width=0.6\columnwidth]{figures/no-sync.png}
\includegraphics[width=0.8\columnwidth]{figures/int-sync.png}
\includegraphics[width=0.8\columnwidth]{figures/full-sync.png}
\caption{3 Control Modes: The Stewart platform introduces a periodic lateral disturbance to the cutting, and this couples with a random control latency. We consider three control architectures: No Synchronization (which executes open-loop), Intermittent Synchronization (which gates the controls to apply at low-velocity periods), and full synchronization (which tracks the motion of the platform exactly). \label{open-loop} }
\end{figure}
\fi


\subsection{3 Control Modes}
%We compare 3 control modes.

\subsubsection{No Synchronization (Open Loop)}
The baseline approach is an open-loop control strategy that cuts along a fixed trajectory. This ignores motion from the Stewart platform. 

\subsubsection{Full Synchronization (Full Tracking)}
%To translate or rotate the cutting arm to compensate for the motion. The natural first choice of controller is a tracking controller--one that models the motion and tries to exactly compensate for it. 
The next approach tracks the motion of the trajectory and tries to compensate for it.
We consider motion estimation, a two-step process where first the system learns a motion model, then uses that motion model to predict a translational offset. To learn the motion model, we observe the motion \todo{explain} of the Stewart platform at 15 fps for 1 minute. We track a colored circle marker \todo{explain} tracked with standard OpenCV circle detection on the platform with an endoscopic stereo camera, and register the stereo frame to an $x$, $y$, $z$ in a fixed global coordinate frame.
Then, in each dimension, we fit a curve:
\[C(t) = \sin (\omega (t + \phi) ) \]
At any point in time, we correct the robot's commanded motion in each dimension with these offsets:
\[
X_{corr}(t) = X_{comm}(t) - C_X(t) %~~~y_{corr} = y_{comm} - C_y~~~z_{corr} = z_{comm} - C_z
\]
where $X$ represents the state space variables for position ($x$, $y$, $z$).

%\subsubsection{Limitations in Tracking Controls} 
Under a quasi-static approximation (which is reasonable for our speed), the tracking controller is an efficient solution and has been widely applied in prior work~\cite{cavusoglu2005control, duindam2007geometric, riviere2006robotic, moustris2013active}. However,
it is quite hard to implement in a physical setup. This requires precise estimation of $\omega, \phi$ from data. Furthermore, it assumes that commands can be sent instantaneously to the robot. 

In practice, the frequency is estimated during experimentation by first taking an endoscope image when the platform reaches a low velocity window and then measuring the average of return times to the selected image.
We find that in 10 cutting trials, the estimated frequency has a relative root-mean-square error (RMSE) of $3\%$ in estimating the period due to kinematic variation in the platform and noise in the images. Furthermore, the phase has an RMSE of $0.22$ seconds due to the frame rate of the camera and noise in the images. If we assume that these errors compound at the worst possible time in the trajectory, namely, when $\frac{d}{dt} =1$, then this noise alone could result in $\approx 1$ mm of RMSE. 
Furthermore, we found that the total execution time varied by 0.576 seconds in latency on any particular cut.
This makes it challenging to time the DVRK to a rhythmic motion.
If this error occurred at the worst time ($\frac{d}{dt} =1$), this would result in an additional $> 3$ mm of error.


\subsubsection{Intermittent Synchronization} 
The results from Figure \ref{dataDBoyd} show the expert surgeon did not try to exactly track the movement.
Instead, he waited for windows of low velocity in the motion, corresponding to the maxima or minima of the sinusoid.
The gauze is deformable and can tolerate some stretching and tension, so the gripper can wait in place as it moves.
Inspired by this, we developed an \emph{intermittent synchronization controller}.

As before, this is a two-step process where first we learn a motion model by fitting a sinusoid to tracking data.
Then, instead of correcting for the motion, we move the robot only during a window of 0.25 seconds around the estimated minima or maxima of the sinusoid.
%Practically, we queue desired cuts and execute only when the robot is available during an open window.
While this controller is sub-optimal, in time we hypothesize that it is more robust to estimation and control errors.
For a sinusoid, the change in position is smallest around the optima $\frac{d}{dt} \approx 0$.
In this window, the uncertainty affects the motion the least.
This basic idea actually applies more generally for any smooth continuous disturbance function. For any function, $\frac{d}{dt} \approx 0$ around the optima. The second derivative around the optima ($\frac{d^2}{d^2t}$) can be used to estimate window width. %
%determines how large the window should be. For some ``pointy'' optima, the window might have to be very small. Therefore, rather than accurately estimating the disturbance, one only needs to know where the optima resides in some window.

\fi

==> dump-arch.tex <==
\section{Problem Statement and Overview}
In this section, we overview the system architecture, assumptions, and inputs and outputs of each component.

\subsection{Problem Statement}
We consider a generalization pattern cutting tasks from Fundamentals of Laparoscopic Surgery (FLS), which is a standard training regimen for medical students in laparoscopic surgery~\cite{Ritter2007}. A typical pattern cutting task features a 50~mm diameter, 2~mm thick circular pattern marked on a 4$\times$4~inch square of standard surgical gauze suspended by clips and that it lies in the horizontal plane. 
We consider a generalization where the gauze is marked with an arbitrary curve that does not self-intersect.

We assume that one arm of the robot is designated as the cutting arm and one is the tensioning arm.
The tensioning arm applies tension to the gauze from a fixed grasping point.
The task is complete once the pattern has been cut from the surrounding gauze.

\subsection{Algorithm Overview}

\begin{enumerate}
    \item \textbf{Inputs: } Parametric planar curve $c(t)$
    
    \item \textbf{Outputs: } Cutting Trajectory $k(t)$, Grasping Points $(x,y)$, Tensioning Policy $\pi$
\end{enumerate}




\vspace{0.25em}

\noindent\textbf{1. Generate Cutting Paths: } Given the registered pattern, represented parametrically by a finite sequence of points, and the kinematic constraints of the da Vinci arm, we automatically generate a fully executable path for cutting. Depending on the pattern, this reachable trajectory may be composed of separate segments such that few temporally adjacent points in the trajectory are non-contiguous. Our heuristic divides the original pattern into segments by determining notch points, or the locations on the pattern where the scissors must begin a new cut, and end points. 

Let us initially assume (will relax subsequently) that the tensioning point is given.
Given this cutting trajectory a first approach would be to always tension orthogonally to the cut.
However, as more of the gauze is cut, the fabric will transfer the tension along multiple distinct paths--making it hard to predict the effect of the tension at the point of cut.
\todo{We highlight this point in our simulated experiments, where we find that on some curves the orthogonal tensioning performs worse than no tensioning at all.}
The tensioning policy needs to be aware of the gauze's deformation and the current progress of the cutting arm.
Since this deformation is difficult to model analytically, Reinforcement Learning (RL) is a viable option.
However, the number of trials run in exploration can be very high, which may not be practical in Patter Cutting because of the cost of resetting failed trials.  
This paper explores the feasibility of a fabric simulator to train an adaptive tensioning policy.

For a tensioning policy and cut trajectory pair, the simulator returns a quality score using the symmetric difference.
Let $X$ be the set of points inside a closed intended trajectory and let $Y$ be the set of points inside a closed simulated trajectory. The symmetric difference is then simply the exclusive-or $A \oplus B$ of the two sets. Open curves are treated as closed curves by forming boundaries with the edges of the cloth.

We can use this quality score to select a grasping point.
We try many random grasping points calculate the tensioning policy and cut trajectory pair and evaluate the quality score with the simulator and select the grasp point that leads to the highest score overall.
\todo{We evaluated learned tensioning policy in physical experiments on the  da Vinci Research Kit (DVRK). 
The simulator is registered to the gauze using colored fiducial points tracked with a computer vision system.}





==> simulator.tex <==

\section{Simulator}
\label{simulator}
A planar fabric can be modeled as a rectangular mesh of vertices. 
These vertices move independently in the x,y,z coordinates governed by forced differential equations.
Suppose, each vertex $(i,j)$ of the fabric has coordinates $p_{ij}^{(x)},p_{ij}^{(y)},p_{ij}^{(z)}  \in \mathbf{R}$, and in isolation, each follows the following equations of motion:
\[
\ddot{p}_{ij} = \alpha p_{ij}  + \delta \dot{p}_{ij} + f(t)
\]
The interaction between the vertices is governed by the tensile modulus $\tau$ acting as an ideal spring:
\[
\ddot{p} = \alpha p  + \delta \dot{p} - \sum_{p' \in \text{neighbors}} \tau (p' - p)  + f(t)
\]
To model cutting, we remove a point from the set of vertices.
\[
\ddot{p} = \alpha p  + \delta \dot{p} - \sum_{p' \in \text{neighbors} \land \neg \text{cut}} \tau (p' - p)  + f(t)
\]
To model standard surgical gauze, we use the following parameters $\delta = 0.008$, $\alpha=0.99$, $\tau=1.0$ and $f(t)$ is gravity.
We fit these parameters through trial and error, observing how cutting trajectories deformed in real gauze vs. the simulator.

We use 625 vertices (25 x 25) in our experiments to approximate the physical gauze. Each time step requires an update of each vertex's location due to external forces such as gravity and internal forces represented by the constraints between adjacent vertices. Running this simulator with many iterations in each run is relatively expensive, so we took several steps to maintain a runtime that would allow both suitable approximation of the cloth and fast computation for update steps. 
We compiled our Python code using the Python package Cython to write C extensions. This sped up each run of the simulation by a factor of six, which allowed us to run tens of thousands of simulations in a reasonable amount of time.\todo{sk. explain}. 

%\todo{change to the symmetric difference: To quantify the effectiveness of the trajectory planning and tensioning policy, we implemented a simple scoring scheme. The subset of vertices approximating the given pattern is tagged as \textit{shape points}. An uncut cloth is given an initial score which reflects the number of shape points in the uncut pattern. Once a simulation is complete, meaning the planned trajectory is executed in full, our code generates a final score directly proportional to the number of shape points that have not been separated or, rather, cut from normal unmarked points}. We then attempt to minimize the score, finding the best trajectory and tensioning policy with which it corresponds.

\subsection*{Step 1. Plan Trajectory}


\subsection*{Step 2. Learn Tensioning Policy}
Using the optimal order of segments, we can arrive at a trajectory for the cutting arm $\chi(n)$ for $n \in \{1,...,N\}$.
Now, our goal is to plan a policy for the tensioning arm, such that this trajectory follows the marked curve as closely as possible.
We model the tensioning problem as a Markov Decision process $\mathcal{M}$:
\[
\mathcal{M} = \langle S,A,T(\cdot,\cdot), R(\cdot,\cdot),N \rangle.
\]
The state-space is defined as a four-tuple consisting of the time index of the trajectory and the displacement vector from the original gripper tensioning location, and the actions are 1mm movements in each of the cardinal directions.
The reward function is the indicator function:
\[
R(s,a) = \mathbf{I}(\chi(n))
\]
which measures whether the next cut applied in the trajectory lands on a marked point on the curve.
The objective is to find a policy $\pi: S \mapsto A$ that optimizes this reward function.

\subsection*{Step 3. Execute}
The da Vinci Research Kit (DVRK) is a development
platform provided by Intuitive Surgical to advance research in teleoperated robotic surgical systems. We use two tools: the Large Needle Driver and the Curved Scissors.
The Large Needle Driver is a grasper with 6 mm fingers (tensioning arm).
The Curved Scissors are a cutting instrument 10 mm in length (cutting arm).
Given the plan $\chi(n)$  and the tensioning policy $\pi$, we execute this on the robot.
Of course, the simulator is an approximation of the true model and the actual execution of the policy on the real gauze will differ from the simulation.
To address this problem, we apply visual position control in addition to the tensioning policy.
